In-sensor 24 classes HAR under 850 Bytes

The year 2023 was a key year for tinyML unleashing a new age of intelligent sensors pushing intelligence from the MCU into the source of the data at the sensor level, enabling them to perform sophisticated algorithms and machine learning models in real-time. This study presents an innovative approach to Human Activity Recognition (HAR) using Intelligent Sensor Processing Units (ISPUs), demonstrating the feasibility of deploying complex machine learning models directly on ultra-constrained sensor hardware. We developed a 24-class HAR model achieving 85\% accuracy while operating within an 850-byte stack memory limit. The model processes accelerometer and gyroscope data in real time, reducing latency, enhancing data privacy, and consuming only 0.5 mA of power. To address memory constraints, we employed incremental class injection and feature optimization techniques, enabling scalability without compromising performance. This work underscores the transformative potential of on-sensor processing for applications in healthcare, predictive maintenance, and smart environments, while introducing a publicly available, diverse HAR dataset for further research. Future efforts will explore advanced compression techniques and broader IoT integration to push the boundaries of TinyML on constrained devices.

==> sections/buffer.tex <==











\section{Real-World Testing and Issues}

In real-world applications, the Intelligent Sensor Processing Unit (ISPU) demonstrated effective performance characterized by an inference time of 150 milliseconds for each 1.5-second data window. This rapid inference capability enables the system to remain inactive approximately 90\% of the time, thereby significantly conserving energy—a critical advantage for battery-powered and energy-constrained environments typical of TinyML deployments. The periods of inactivity present opportunities for the ISPU to perform additional computational tasks without impacting the primary classification functions. These tasks could include spectral analysis and advanced feature extraction, which may enhance the system’s overall functionality and provide deeper insights into the sensor data. By efficiently managing active and inactive states, the ISPU not only optimizes energy usage but also allows for the integration of more sophisticated processing techniques during idle periods, thereby expanding the potential applications and improving the robustness of machine learning models within the TinyML framework.



\section{Discarded and Merged Classes}
During the incremental class injection process, certain classes were either discarded or merged to enhance model performance and maintain memory efficiency. The "Brushing Teeth" class was discarded due to a high incidence of false positives with other classes within the cleaning category, such as "Brushing Hair," "Washing Face," and "Shaving." This misclassification was primarily attributed to the need for specific gyroscope calibration, as the high-frequency motions involved in brushing teeth differed significantly from those of other cleaning activities. Additionally, the "Driving" class was excluded because it lacked periodic movement within the selected window size, and the random acceleration and braking associated with driving introduced unpredictable spikes in the data. Furthermore, when a vehicle was moving at a relatively constant speed on a straight road, the system erroneously classified it as handstill based on the principle of inertia.
On the other hand, certain classes were merged to improve classification stability and reduce confusion. For instance, the "Writing" class exhibited misclassifications between return movements and forward movements, which were resolved by combining them into a single class. Similarly, the "Writing on Board" class showed enhanced stability when merged with the general "Writing" class. The "Using Computer" class also benefited from merging, as it initially caused the model to switch randomly between two distinct classes. By consolidating these classes, the model's reliability and accuracy were significantly improved. These adjustments—discarding problematic classes and merging similar ones—were crucial in maintaining a cohesive and efficient class structure, thereby ensuring the robustness and scalability of the TinyML framework.

\section{tradeoff}
The tradeoff between accuracy and the number of classes illustrates the model’s capability to sustain relatively high accuracy levels even as the number of classification categories increases, thereby emphasizing its scalability. Typically, an expansion in the number of classes can lead to a decline in model accuracy due to heightened complexity and the potential for greater class overlap. However, in this study, the model demonstrates a robust ability to maintain performance metrics despite the growing number of classes. This achievement is attributed to the implementation of an incremental class injection strategy, which effectively manages class boundaries and minimizes confusion among similar categories. The ability to uphold high accuracy while accommodating an increasing number of classes is crucial for practical applications of TinyML, where resource constraints and the need for efficient processing are paramount. Consequently, this balance not only validates the model’s scalability but also reinforces its suitability for deployment in diverse and dynamically evolving environments. These findings underscore the model’s robustness and adaptability, making it a viable solution for complex classification tasks within the TinyML framework.


